First-Order Bilevel Topology Optimization for Fast Mechanical Design

Topology Optimization (TO), which maximizes structural robustness under material weight constraints, is becoming an essential step for the automatic design of mechanical parts. However, existing TO algorithms use the Finite Element Analysis (FEA) that requires massive computational resources. We present a novel TO algorithm that incurs a much lower iterative cost. Unlike conventional methods that require exact inversions of large FEA system matrices at every iteration, we reformulate the problem as a bilevel optimization that can be solved using a first-order algorithm and only inverts the system matrix approximately. As a result, our method incurs a low iterative cost, and users can preview the TO results interactively for fast design updates. Theoretical convergence analysis and numerical experiments are conducted to verify our effectiveness. We further discuss extensions to use high-performance preconditioners and fine-grained parallelism on the Graphics Processing Unit (GPU).

==> old/conclusion.tex <==
Our initial investigations of bilevel TO optimization open doors to several avenues of extensions to more complex problem settings. A useful extension would consider uncertain external loads via game theory \cite{holmberg2017game}, which could prepare the mechanical system for more general use cases. Although our method can account for multiple external load configurations, each configuration is treated equally. Instead, \citewithauthor{holmberg2017game} actively search for the worst-case loads via a zero-sum game, leading to more robust designs. Accounting for strain/stress limits poses another important direction. When these limits are violated, certain materials can be locally damaged even when the structure is globally strong. But these constraints can be extremely challenging to incorporate because they are non-convex in both $u$ and $v$. Finally, the recent research \cite{shaban2019truncated} on bilevel solvers with non-convex low-level problems lies the foundation for TO governed by large deformations \cite{buhl2000stiffness,bruns2001topology}. Large deformations are essential when optimizing for soft materials. \kui{what are you trying to say here?}

==> old/experiments.tex <==
On the third row, we plot the evolution of high- and low-level errors over iterations. Clearly, the low-level tracking error quickly reduces to satisfy the second stopping condition and our algorithms are almost always trying to satisfy the high-level stopping condition. This observation empirically justifies our choice of approximate matrix inversion, because the error due to such approximation vanishes quickly.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth, height=0.5\linewidth]{figs/placeholder.png}
\caption{\label{fig:preconCompare} \small{The convergence history of \prettyref{alg:CPOpt} with a Krylov-preconditioner, measured by the relative infill level change. Overall, we find that choosing $D=\TODO{XXX}$ achieves the best overall performance in terms of computational cost.}}
\vspace{-10px}
\end{figure}
We first compare FBTO with and without preconditioner on the benchmark from \prettyref{fig:teaser}. We choose to use the Krylov-preconditioner for \prettyref{alg:CPOpt} with $D=20$, unless otherwise stated. In \prettyref{fig:history}, the convergence history of the two versions is plotted against both iteration number and computational time. The preconditioner can significantly boost our convergence rate and save computation and we further compare the performance under different choices of $D$ in \prettyref{fig:preconCompare}. Overall, we find the using $D=\TODO{XXX}$ achieves the best performance in terms of computational time. For whatever choice of algorithm and parameter $D$, the cost of each FBTO iteration is below $\TODO{XXX}$ms, which allows a robot designer to quickly experiment with different parameters and preview results to refine the design.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth, height=0.5\linewidth]{figs/placeholder.png}
\caption{\label{fig:exactSolve} \small{We compare the convergence rate of the high-level problem with exact and inexact matrix inversions. As expected, the small convergence rate boost does not justify the high cost of exact matrix inversions.}}
\vspace{-10px}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth, height=0.5\linewidth]{figs/placeholder.png}
\caption{\label{fig:compareSQP} \small{We compare the convergence rate and iterative cost of FBTO and SQP. The solve time of SQP grows superlinearly with $E$, while our method exhibits a linear growth of computation.}}
\vspace{-10px}
\end{figure}
We then compare our method with two baseline algorithms. Our first baseline replaces the first step of \prettyref{alg:Opt} with an inner loop to exactly solve the low-level problem during each bilevel iteration. As plotted in \prettyref{fig:exactSolve}, this strategy only brings marginal boost to the convergence rate, which comes at a much higher iterative cost. As pointed out above, this is because our algorithm is mostly focused on solving the high-level problem, while the low-level tracking error is typically small. Therefore, using much computational resource to further reduce the already small tracking error would have diminishing return. Our second baseline is the off-the-shelf SQP solver \cite{gill2005snopt}, which requires exact matrix inversion for computing the objective function value in the line search and the exact gradient direction. We use the same stopping criteria for the two algorithms and compare their wall time to solve the same problem in \prettyref{fig:teaser}. As illustrated \prettyref{fig:compareSQP}, the solve time of SQP quickly grows with $E$, while our method can handle these problems with a low iterative and overall cost.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth, height=0.5\linewidth]{figs/placeholder.png}
\caption{\label{fig:resolution} \small{We plot the number of iterations and computational time until convergence of \prettyref{alg:CPOpt} against different grid resolutions.}}
\vspace{-10px}
\end{figure}
Finally, we investigation the influence of grid resolutions on the algorithm's convergence rate. Again for the problem in \prettyref{fig:teaser}, we solve it by \prettyref{alg:CPOpt} under a row of different grid resolutions and plot the required iteration count and computational time in \prettyref{fig:resolution}. The number of iterations grows superlinearly with the resolution. We expect certain preconditioners can accelerate information spreading and make the iteration count roughly independent of grid resolutions. One promising choice is the multigrid preconditioner.


